Realtime Time Synchronized Event-based Stereo

In this work, we propose a novel event based stereo method which addresses the problem of motion blur for a moving event camera. Our method uses the velocity of the camera and a range of disparities to synchronize the positions of the events, as if they were captured at a single point in time. We represent these events using a pair of novel time synchronized event disparity volumes, which we show remove motion blur for pixels at the correct disparity in the volume, while further blurring pixels at the wrong disparity. We then apply a novel matching cost over these time synchronized event disparity volumes, which both rewards similarity between the volumes while penalizing blurriness. We show that our method outperforms more expensive, smoothing based event stereo methods, by evaluating on the Multi Vehicle Stereo Event Camera dataset.

==> tex/Algorithm.tex <==
\begin{algorithm}
\caption{Event-based Stereo Depth by Defocus}\label{algorithm}
\small
\algblock[Name]{Input}{EndInput}
\algblock[Name]{StereoDisparity}{EndStereoDisparity}
\algtext*{EndInput}
\algtext*{EndStereoDisparity}
\algrenewtext{StereoDisparity}{\textbf{Stereo Disparity Estimation}}
\begin{algorithmic}[0]
\Input
\State Camera linear and angular velocity, $\mathbf{v},\boldsymbol{\omega}$.
\State Left and right events, $\{(x_i, y_i, t_i, p_i)\}_{L, R}$.
\EndInput
\StereoDisparity
\State Estimate the shifted event position for each event and each disparity using \eqref{eq:time_shift}.
\State Generate the left and right event disparity volumes $I_{L}$ and $I_{R}$ using \eqref{eq:left_event_image} and \eqref{eq:right_event_image}.
\State Calculate the union cost $I_{L}\cup I_{R}$ \eqref{eq:union_cost}.
\State Calculate the intersection cost $I_{L}\cap I_{R}$ \eqref{eq:intersection_cost}.
\State Calculate the full cost volume \eqref{eq:total_cost}.
\EndStereoDisparity
\end{algorithmic}
\label{alg:algorithm}
\end{algorithm}

==> tex/ErrFigs.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/disparity_one2_cop.png}
\caption*{CopNet err. $<$ 1 pix.}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/disparity_two2_cop.png}
\caption*{CopNet err. $<$ 2 pix.}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/disparity_one2_our.png}  
\caption*{TSES err. $<$ 1 pix.}
\end{subfigure}
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\linewidth]{figs/disparity_two2_our.png}  
\caption*{TSES err. $<$ 2 pix.}
\end{subfigure}
  \caption{Sample visualization of the error distribution of CopNet vs TSES. Disparities with error less than the specified tolerance (1 or 2 pix.) are displayed. Best viewed in color.}
  \label{fig:errs}
\end{figure}
